ItTakesTwo: Leveraging Peer Representations for Semi-supervised LiDAR Semantic Segmentation

The costly and time-consuming annotation process to produce large training sets for modelling semantic LiDAR segmentation methods has motivated the development of semi-supervised learning (SSL) methods. However, such SSL approaches often concentrate on employing consistency learning only for individual LiDAR representations. This narrow focus results in limited perturbations that generally fail to enable effective consistency learning. Additionally, these SSL approaches employ contrastive learning based on the sampling from a limited set of positive and negative embedding samples. This paper introduces a novel semi-supervised LiDAR semantic segmentation framework called ItTakesTwo (IT2). IT2 is designed to ensure consistent predictions from peer LiDAR representations, thereby improving the perturbation effectiveness in consistency learning. Furthermore, our contrastive learning employs informative samples drawn from a distribution of positive and negative embeddings learned from the entire training set. Results on public benchmarks show that our approach achieves remarkable improvements over the previous state-of-the-art (SOTA) methods in the field. The code is available at: https://github.com/yyliu01/IT2.

==> rebuttal/lasermix_ablation.tex <==
\begin{table}[t!]
\caption{Comparison between our IT2 and LaserMix with our contrastive learning (i.e., ctrs.) on the nuScenes dataset based on voxel representation. Our results are highlighted in \textcolor{darkred}{red}.}
\label{tab:rebuttal_lasermix}
\centering
\resizebox{.3\textwidth}{!}{
\begin{tabular}{c|cc}
\specialrule{1pt}{0pt}{0pt}
\multirow{2}{*}{Method} & \multicolumn{2}{c}{nuScenes} \\
\cline{2-3}
                        & 1\%     & 10\%       \\
\hline
LaserMix~\citelasermix          &   55.3      &   69.9         \\
\hline
LaserMix+ctrs.          &    56.2     &   71.0          \\
IT2                     &   \textcolor{darkred}{57.5} \textcolor{gray}{(1.3$\uparrow$)}      &   \textcolor{darkred}{72.1} \textcolor{gray}{(1.1$\uparrow$)}          \\
\specialrule{1pt}{0pt}{0pt}
\end{tabular}}
\vspace{-15pt}
\end{table}

% \begin{table}[t!]
% \caption{Comparison between our methods and LaserMix with contrastive learning (i.e., ctrs.) on the nuScenes dataset based on voxel representation. Our results are highlighted in \textcolor{darkred}{red}.}
% \label{tab:rebuttal_lasermix}
% \centering
% \resizebox{.3\textwidth}{!}{
% \begin{tabular}{c|ccc}
% \specialrule{1pt}{0pt}{0pt}
% \multirow{2}{*}{Method} & \multicolumn{3}{c}{nuScenes} \\
% \cline{2-4}
%                         & 1\%     & 10\%     & 20\%    \\
% \hline
% LaserMix          &   55.3      &   69.9        &    71.8     \\
% \hline
% LaserMix+ctrs.          &    56.2     &   71.0     &         \\
% IT2                     &   57.5      &   72.1       &   73.6      \\
% \specialrule{1pt}{0pt}{0pt}
% \end{tabular}}
% \vspace{-15pt}
% \end{table}


% \begin{table}[t!]
% \caption{Comparison between our methods and LaserMix on the nuScenes dataset. `MT' denotes the Mean Teacher framework, and the $\dagger$ symbol indicates that the results are from LaserMix. The results with other contributions are highlighted in \textcolor{darkred}{red}.}
% \centering
% \resizebox{.4\textwidth}{!}{\begin{tabular}{c|cc|cc}
% \specialrule{1pt}{0pt}{0pt}
% Repr.        & \multicolumn{2}{c|}{range} & \multicolumn{2}{c}{voxel} \\
% \hline
% ratio        & 10\%    & 20\%      & 10\%    & 20\%     \\
% \specialrule{1pt}{0pt}{0pt}
% MT$\dagger$           &     60.4    &  65.4           &    66.0       &     67.1        \\
% IT2          &    67.3      &  70.8       &    70.4     &  71.9          \\
% \hline
% MT+LaserMix$\dagger$   &    68.2       & 70.6          &    69.9      &    71.8        \\
% IT2+LaserMix &        &                   &        &        \\
% \hline
% IT2 {\small + our other contributions}         &   \textcolor{darkred}{71.3}      &   \textcolor{darkred}{73.4}         &    \textcolor{darkred}{72.1}     &    \textcolor{darkred}{73.6}         \\
% \specialrule{1pt}{0pt}{0pt}    
% \end{tabular}}
% \vspace{-15pt}
% \end{table}

% \begin{table}[t!]
% \caption{Comparison between our methods and LaserMix on the nuScenes dataset. `MT' denotes the Mean Teacher framework, and the $\dagger$ symbol indicates that the results are from LaserMix. The results with other contributions are highlighted }
% \resizebox{.5\textwidth}{!}{\begin{tabular}{c|ccc|ccc}
% \specialrule{1pt}{0pt}{0pt}
% Repr.        & \multicolumn{3}{c|}{range} & \multicolumn{3}{c}{voxel} \\
% \hline
% ratio        & 10\%    & 20\%   & 50\%   & 10\%    & 20\%   & 50\%   \\
% \specialrule{1pt}{0pt}{0pt}
% MT$\dagger$           &     60.4    &  65.4      &  69.4        &    66.0       &     67.1    &  71.7      \\
% IT2          &    67.3      &  70.8      &  72.6      &    70.4     &  71.9      &  73.1      \\
% \hline
% MT+LaserMix$\dagger$   &    68.2       & 70.6          &   73.0       &    69.9      &    71.8    & 73.2       \\
% IT2+LaserMix &        &     &       &         &        &        \\
% \hline
% Ours         &   71.3      &   73.4     &  74.0      &    72.1     &    73.6    &   74.1     \\
% \specialrule{1pt}{0pt}{0pt}    
% \end{tabular}}
% \vspace{-15pt}
% \end{table}



==> rebuttal/m_ablation.tex <==
\begin{table}[t!]
\caption{\textbf{Ablation study of Components (M)} in Gaussian Mixure Model (GMM) on the nuScenes dataset under the 10\% labelled data protocol. The best results are highlighted in \textcolor{darkred}{red}.}
\centering
\label{tab:rebuttal_component}
\resizebox{.35\textwidth}{!}{\begin{tabular}{c|cccc}
\specialrule{1pt}{0pt}{0pt}
\multicolumn{5}{c}{nuScenes (with 10\% labelled data)} \\
\hline
Component (M)     & M=1     & M=3       & M=5    & M=7    \\
range Repr.       & 70.4  & 70.8       &    \textcolor{darkred}{71.3}    & 71.2         \\
voxel Repr.       & 71.4   & 71.7       &    \textcolor{darkred}{72.1}   & 71.9         \\
\specialrule{1pt}{0pt}{0pt}
\end{tabular}}
\vspace{-15pt}
\end{table}

==> rebuttal/temp_ablation.tex <==
\begin{table}[t!]
\caption{Ablation study of different \textbf{temperature (Temp.)} values comparing our methods with ContrasSeg~\citectrsseg~on the nuScenes dataset, under the 10\% labelled data protocol. The best results for both methods are highlighted in \textcolor{darkred}{red}.}
% \gustavo{Could you add one more temperature value (maybe t=0.15)?} \yy{Yes, will do.}
\label{tab:rebuttal_temp}
\centering
\resizebox{.38\textwidth}{!}{\begin{tabular}{c|ccc|ccc}
\specialrule{1pt}{0pt}{0pt}
Repr.     & \multicolumn{3}{c|}{range} & \multicolumn{3}{c}{voxel} \\
\hline
Temp. (t) & t=0.05  &  t=0.10 & t=0.15 & t=0.05  & t=0.10 & t=0.15 \\
\hline
ContrasSeg~\citectrsseg   &     69.4            &      \textcolor{darkred}{70.3}  &  69.3 &  70.1            &   \textcolor{darkred}{71.2}    &  70.5 \\
Ours      &  70.3           &   \textcolor{darkred}{71.3}   &  70.4 &   71.0          &  \textcolor{darkred}{72.1}  &     71.5 \\
\specialrule{1pt}{0pt}{0pt}
\end{tabular}}
\vspace{-15pt}
\end{table}

% \begin{table}[t!]
% \caption{Ablation study of different \textbf{temperature} values comparing our methods with ContrasSeg on the nuScenes dataset, under the 10\% labelled data protocol. \gustavo{Could you add one more temperature value (maybe t=0.15)?} \yy{Yes, will do.}}
% \label{tab:rebuttal_temp}
% \centering
% \resizebox{.35\textwidth}{!}{\begin{tabular}{c|cc|cc}
% \specialrule{1pt}{0pt}{0pt}
% Repr.     & \multicolumn{2}{c|}{range} & \multicolumn{2}{c}{voxel} \\
% \hline
% Temp. (t) & t=0.05  & t=0.10 & t=0.05  & t=0.10 \\
% \hline
% supCons   &     69.4            &      70.3  &    70.1            &   71.2     \\
% Ours      &  70.3           &   71.3     &   71.0          &  72.1      \\
% \specialrule{1pt}{0pt}{0pt}
% \end{tabular}}
% \vspace{-15pt}
% \end{table}

% \begin{table}[t!]
% \caption{Ablation study of \textbf{temperature} in nuScenes dataset with \ul{10\% labelled data} protocol.}
% \label{tab:rebuttal_temp}
% \resizebox{.5\textwidth}{!}{\begin{tabular}{c|ccc|ccc}
% \specialrule{1pt}{0pt}{0pt}
% Repr.     & \multicolumn{3}{c|}{range} & \multicolumn{3}{c}{voxel} \\
% \hline
% Temp. (t) & t=0.05  & t=0.07 & t=0.10 & t=0.05  & t=0.07 & t=0.10 \\
% \hline
% supCons   &     69.4    &        &      70.3  &    70.1     &        &   71.2     \\
% Ours      &  70.3       &   70.8     &   71.3     &   71.0      &   71.8     &  72.1      \\
% \specialrule{1pt}{0pt}{0pt}
% \end{tabular}}
% \end{table}



==> sections/0_abstract.tex <==
\begin{abstract}
The costly and time-consuming annotation process to produce large training sets for modelling semantic LiDAR segmentation methods has motivated the development of semi-supervised learning (SSL) methods. 
% One of the primary components in such SSL methods is the consistency learning that has demonstrated promising performance by encouraging the consistent prediction across various input perturbations. 
% Even though successful, these SSL methods have not harnessed the multiple transformed views or peer representations of the outdoor LiDAR data and, instead, applied  consistency learning only to single LiDAR representations, leading to two potential issues:
% 1) the impact of perturbations applied to  single representations is limited; and 
% 2) different representations possess distinct strengths and weaknesses for handling SSL problems.
While these SSL methods have achieved success, they have yet to fully leverage the complementarity inherent in multiple transformed views or peer representations of outdoor LiDAR data. Instead, they have predominantly focused on applying consistency learning only to individual LiDAR representations. This approach has led to a limited exploration of perturbations applied to single representations, constraining the potential benefits of incorporating diverse representations.
% In addition, previous approaches utilise contrastive learning based on the limited sampling from a finite set of positive and negative embedding samples, instead of considering the sampling from a more holistic distribution of positive and negative embeddings.
Additionally, these SSL approaches employ contrastive learning based on the restricted sampling from a finite set of positive and negative embedding samples, rather than considering a more effective sampling from a distribution of positive and negative embeddings.
% In addition, even though contrastive learning has also been used to produce competitive SSL LiDAR segmentation methods, previous approaches explored quite limited sampling techniques to produce the positive and negative samples by ignoring a more holistic distribution of the embedding in the feature space. \\
% In this paper, we propose the ItTakesTwo (IT2) method, a new semi-supervised LiDAR semantic segmentation method that enforces consistent predictions from peer LiDAR representations.
% In this paper, we propose the novel semi-supervised LiDAR semantic segmentation framework ItTakesTwo (IT2), which enforces consistent predictions from peer LiDAR representations to enhance the perturbation effectiveness of the consistency learning.
% Furthermore, our model is trained with contrastive learning using informative positive and negative samples drawn from a  distribution of the feature space learned from the whole training set.
This paper introduces a novel semi-supervised LiDAR semantic segmentation framework called ItTakesTwo (IT2). IT2 is designed to ensure consistent predictions from peer LiDAR representations, thereby improving the perturbation effectiveness in consistency learning. Furthermore, our contrastive learning employs informative samples drawn from a distribution of positive and negative embeddings learned from the entire training set.
% Also, while previous works utilise the same augmentation functions for different LiDAR representations, we have observed that employing innovative representation-specific augmentation functions enhance the generalisation of our method.
Results on public benchmarks show that our approach achieves remarkable improvements over the previous state-of-the-art (SOTA) methods in the field. \textcolor{red}{Code will be available.} 

\end{abstract}

==> sections/1_introduction.tex <==
\section{Introduction}
\label{sec:introduction}
Outdoor LiDAR semantic segmentation is emerging as an important area of research given its application to self-driving vehicles~\cite{grigorescu2020survey,guo2020deep}. Offering unique challenges, such as data sparsity~\cite{zhu2021cylindrical} and varying point density~\cite{kong2023lasermix,milioto2019rangenet++}, most of the existing works address those issues by transforming those LiDAR points to other representations, including range-based images~\cite{wu2018squeezeseg,kong2023rethinking,fan2021rangedet,milioto2019rangenet++}, voxel grids~\cite{graham20183d,zhu2021cylindrical,hou2022point}, or fusing the LiDAR points with multiple modalities~\cite{liu2023bevfusion, liu2023segment} and views~\cite{xu2021rpvnet}. 
Despite their success, those methods are based on supervised learning strategies that require large labelled training sets, which is problematic given the costly and time-consuming labelling process~\cite{liu2022perturbed,ouali2020semi}.

\begin{figure}[t!]
    \centering
    \includegraphics[width=\textwidth]{images/first_page_demonstration.pdf}
    \caption{The \textbf{left} figure displays the 3D point cloud scan (ground truth) and the \textbf{right} figures show the transformed \textcolor{rangered}{range (top-right)} and \textcolor{voxelblue}{voxel (bottom-right)} representations with the predictions from the range and voxel models \gustavo{Yuyuan, please add the models in the figure}. 
    % \gustavo{why do we need to say ground truth and pseudo labels in this image?} \yy{because the left figure is the ground truth results, and the right figures are the predictions. We need to highlight they have complementary performance for different categories.}, 
    %where the incorrect predictions are marked in \textcolor{gray}{gray}. 
    % \gustavo{these gray regions are hard to see...} \yy{well, should we simply don't mention that? because it is not that important.}. 
    Notice how the same categories, such as Terrain (\terrain),  can be transformed between representations. 
    Also note the different results produced by the range and voxel models, depicted in the histograms of  segmentation predictions on the right hand side. Such differences demonstrate the potential complementarity of the peer representations' predictions.
    \gustavo{the gray regions can be erased. I don't know how to introduce the equations $y_{point}$... suggest to remove it.}
    %share \ul{consistent} semantic meaning and also own \ul{complementary} pseudo label qualities. 
    % \gustavo{What is the histogram for range and voxel?} \yy{It demonstrates the IoU results for different categories.} 
    % \gustavo{What is the point of this figure? Is it to show the complementarity of the two modalities? The red and blue arrows need to be clearly marked with range and voxel. Also, what are the $y_{point} \Longrightarrow y_{pixel}$? Are they needed?} \yy{I'm trying to say the point in the left figure are transfered to the range (top) and voxel (bottom) with these arrows. The identical mark shows they own unique semantic meaning.}
    % \gustavo{The main thing I see from this figure is the transformation from point cloud to range and volumetric. I don't see much information about the complementarity of the the modalities.  I also don't think we should talk about pseudo-labels or classification here since I don't see any model anywhere in the figure. So we don't mention pseudo labels and we don't plot the histogram of classification, unless you think it's important to have it here and I'm missing the reason.} \yy{We have discussed that different modalities have different performance in categories, and the histograms demonstrate the results. I can draw the model blocks near the red and blue arrows if that can make things more clear...}
    }
    \label{fig:demo}
    \vspace{-15pt}
\end{figure}

These limitations motivated the development of semi-supervised LiDAR semantic segmentation methods~\cite{kong2023lasermix, jiang2021guided, li2023less}, which are usually based on Mean Teacher (MT)~\cite{tarvainen2017mean} or contrastive learning~\cite{khosla2020supervised} to 
enable the training with labelled and unlabelled data. 
A particularly successful semi-supervised learning (SSL) technique is  consistency learning, which draws upon the Cluster hypothesis\footnote{\protect Cluster hypothesis (or assumption)~\cite{manning2009introduction}: the data with various forms that behave similarly with respect to relevance to information should be clustered together.}. Consistency learning aims to reduce the differences between the perturbed predictions from an input data~\cite{chen2021semi,ouali2020semi}, where the perturbations can be obtained via input augmentation~\cite{yang2021st++,zou2020pseudoseg}, adversarial noise~\cite{liu2022perturbed,hung2018adversarial}, and network perturbations~\cite{chen2021semi,yang2023revisiting}. 
Current LiDAR SSL segmentation methods~\cite{kong2023lasermix,li2023less,jiang2021guided}, employ consistency learning with robust and diverse perturbations but restrict their application to individual LiDAR representations. Typically, perturbations are applied exclusively to either the range view (top-right, marked in \textcolor{rangered}{red}) or the voxel grid (bottom-right, marked in \textcolor{voxelblue}{blue}) as illustrated in Fig.\ref{fig:demo}~\cite{french2019semi, liu2022perturbed, yang2021st++, yang2023revisiting}.
%However, a powerful perturbation method is based on maintaining the prediction consistency between the range and voxel views. For instance, in Fig.~\ref{fig:demo}, the  Terrain (\terrain) elements for both representations are associated with the same 3D point. 
Unfortunately, focusing on only one of the representations is disadvantageous because each representation has significant issues, such as (see Fig.~\ref{fig:demo}): 1) the range view suffers from information loss due to the spherical projection process, particularly for tail categories, like Pole (\pole) which shows only 52.02 mIoU; and 2) the voxel view can have lower accuracy in  dense regions far away from the LiDAR source, e.g., Sidewalk (\sidewalk) with 69.50 mIoU. 
%Hence, the effectiveness of these consistency learning approaches is severely affected by their reliance on a single representation~\cite{kong2023lasermix,li2023less,jiang2021guided}.
A major negative consequence of such mistaken predictions during SSL is that they lead to confirmation bias (i.e., the problem of using wrong predictions for training), which tends to detract the whole training process.
%these issues is that the presence of erroneous pseudo-labels in specific categories not only hampers performance during training but is also likely to induce confirmation bias.


% Another successful SSL technique in LiDAR segmentation is contrastive learning~\cite{jiang2021guided,li2023less,cheng2021sspc,hou2021exploring}, which consists of forming positive and negative embedding pairs at instance~\cite{nunes2022segcontrast} or category~\cite{jiang2021guided,li2023less} levels, thereby improving the the latent space representation.
% To form such positive and negative embedding pairs, those methods rely on a limited amount of \ul{random samples} extracted from the training sample embeddings.  This amount is limited due to computational resource limitations~\cite{jiang2021guided,li2023less}.
% Unfortunately, such limited amount of samples prevents a holistic understanding of the distribution across the entire embedding space~\cite{caron2020unsupervised}, leading to a sub-optimal SSL optimisation. 
% This issue is particularly pronounced when dealing with embeddings from different networks in multiple representations or views, where potentially noisy data~\cite{miech2020end,tian2020contrastive} or model bias~\cite{xu2022multi} from one network can negatively impact the others, further hindering the optimisation process.
Another effective SSL technique for LiDAR segmentation is contrastive learning~\cite{jiang2021guided,li2023less,cheng2021sspc,hou2021exploring}. This method involves creating positive and negative embedding pairs at the instance~\cite{nunes2022segcontrast} or category~\cite{jiang2021guided,li2023less} levels, thereby enhancing the latent space representation. However, to generate these pairs, the methods rely on a limited number of random samples extracted from the training sample embeddings due to computational constraints~\cite{jiang2021guided,li2023less}. Unfortunately, this limited sample size hinders a comprehensive understanding of the distribution across the entire embedding space~\cite{caron2020unsupervised}, resulting in suboptimal SSL optimization. This limitation becomes particularly pronounced when dealing with embeddings from different models in multiple views, where potential noisy data~\cite{miech2020end,tian2020contrastive} or model bias~\cite{xu2022multi} from one network can adversely affect others, thereby impeding the optimization process.

To address the research challenges mentioned above, we propose a novel SSL LiDAR segmentation, called ItTakesTwo (IT2). 
%, which relies on enforcing the prediction consistency between two peer LiDAR representations. Our 
IT2 leverages consistency learning with two peer LiDAR representations, enhancing perturbation effectiveness by enforcing prediction consistency between representations. This approach addresses challenges associated with prediction problems arising from single representations.
Furthermore, IT2 introduces a contrastive learning, where 
instead of randomly selecting samples from training embeddings, we learn class prototype distributions (via Gaussian Mixture Models) and sample from it to produce more representative samples that 
%we use the most representative embedding (also known as prototype) with respect to a particular training sample, and enforce the embedding of this sample to be more similar to its corresponding prototype. Such prototypes are represented by Gaussian Mixture Models (GMMs) that are trained to fit the distribution across the entire embedding space from both representations. Consequently, we can sample virtual prototypes from these GMMs and use them for embedding pairs to 
enhance the efficiency  \gustavo{this is vague -- what is meant by efficiency? training time? harder negatives and positives?} \yy{with informative prototype embeddings?} of contrastive learning in peer representation scenarios. 
In addition, instead of applying single type of augmentation to both LiDAR representations~\cite{kong2023lasermix}, we experimentally found that better generalisation can be achieved by applying different augmentation functions to each representation. 
%We thus explore the representation-related strong augmentation for our IT2 architecture. 
To summarise, our work has the following key contributions:
\begin{enumerate}
    \item We propose a novel SSL LiDAR segmentation method (IT2) that encourages consistent predictions from different LiDAR representations;
    \item To enhance the feature-level understanding from multiple LiDAR representations, we introduce GMM models to generate the most representative embedding samples for more effective contrastive learning;
    % \item On top of our architecture, we propose new LiDAR representation specific data augmentation to improve the generalisation of our model.
\end{enumerate}
\gustavo{it doesn't make sense to have the augmentation contribution in the text, but not in the bullet points. Either list in both or don't claim anything} \yy{We can claim it in here, but it is a minor contribution. We can not avoid it, because it brings improvements in our ablation.}
Our IT2 has state-of-the-art (SOTA) performance on nuScenes~\cite{caesar2020nuscenes}, SemanticKitti~\cite{behley2019semantickitti} and ScribbleKitti~\cite{unal2022scribble}, and we also achieve the best performance with different sampling strategies. 
Notably, in nuScenes~\cite{caesar2020nuscenes}, we have outperformed the previous SOTA approach~\cite{kong2023lasermix} by $\sim 2.5\%$ in the limited labelled data situations.



==> tables/table_multi_modality.tex <==
% \begin{table}[]
% \resizebox{\textwidth}{!}{
% \begin{tabular}{ccccccc}
% \multirow{2}{*}{Methods} & \multirow{2}{*}{LiDAR}   & \multirow{2}{*}{Camera} & \multirow{2}{*}{Params.} & \multicolumn{3}{l}{SemanticKITTI} \\
%                          &                          &                        &                          & 1\%       & 5\%       & 10\%      \\
% ImageTo360~\cite{chen2018encoder} {\scriptsize \textcolor{gray}{(ICCV'23 workshop)}}               & Cylinder3D~\cite{zhu2021cylindrical}               & DeepLabV3+~\cite{chen2017deeplab}             &                          &           &           &           \\
% ImageTo3600~\cite{chen2018encoder} {\scriptsize \textcolor{gray}{(ICCV'23 workshop)}}               & Cylinder3D~\cite{zhu2021cylindrical}               & SegFormer~\cite{xie2021segformer}              &                          &           &           &           \\
% lim3D                    & Cylinder3D/Cylinder3D &                        &                          &           &           &           \\
% IT2                      & Cylinder3D \& FidNet     &                        &                          &           &           &          
% \end{tabular}}
% \end{table}

\begin{table*}[t!]
\renewcommand{\arraystretch}{1.1}
\caption{\textbf{Comparison with significant sampling and post-processing methods} results in different partition protocols. In addition, the comparison approaches~\cite{reichardt2023360deg,li2023less} utilise post-process for pseudo-labelling during training. }
\resizebox{\textwidth}{!}{
\begin{tabular}{?c|c|c|c?c|c|c|c?}
\specialrule{1.5pt}{0pt}{0pt}
\multirow{2}{*}{Methods}& \multirow{2}{*}{Post} & \multicolumn{2}{c?}{Modalities}         & \multicolumn{4}{c?}{SemanticKITTI~\cite{behley2019semantickitti}}\\
\cline{3-8}
                         & & LiDAR {\scriptsize (point)}                    & Camera  {\scriptsize (pixel)}   & 5\%    & 10\%   & 20\%   & 40\%                             \\
\specialrule{1.5pt}{0pt}{0pt}
ImageTo360~\cite{reichardt2023360deg}              & train \texttt{\&} valid & Cylinder3D~\cite{zhu2021cylindrical}                & DeepLabV3+~\cite{chen2018encoder} &     58.29   &   58.62     &   61.44     &  -                               \\
ImageTo360~\cite{reichardt2023360deg}             & train \texttt{\&} valid &Cylinder3D~\cite{zhu2021cylindrical}                 & SegFormer~\cite{xie2021segformer}  &    59.26   & 60.00       &  62.27      &  -                               \\
\specialrule{1.5pt}{0pt}{0pt}
Lim3D~\cite{li2023less}                   & \xmark &Cylinder3D~\cite{zhu2021cylindrical} \texttt{\&} Cylinder3D~\cite{zhu2021cylindrical} &   \xmark   &  56.8        &   59.6    &   60.5     &    61.4                               \\IT2 {\scriptsize \textcolor{gray}{(Ours)}}                &   \xmark   & Cylinder3D~\cite{zhu2021cylindrical} \texttt{\&} FidNet~\cite{zhao2021fidnet}       &  \xmark          &  60.30      &   62.63     &        &      63.79    \\
\hline
Lim3D~\cite{li2023less}                    & train \texttt{\&} valid &Cylinder3D~\cite{zhu2021cylindrical} \texttt{\&} Cylinder3D~\cite{zhu2021cylindrical} &   \xmark   &   59.5    &   62.2     &   63.1     &    63.3                                \\IT2 {\scriptsize \textcolor{gray}{(Ours)}}                &   valid   & Cylinder3D~\cite{zhu2021cylindrical} \texttt{\&} FidNet~\cite{zhao2021fidnet}       &  \xmark          &        &        &        &           \\
% Lim3D+SDSC~\cite{li2023less} {\scriptsize \textcolor{gray}{(CVPR'23)}}                    & Cylinder3D~\cite{zhu2021cylindrical} \texttt{\&} Cylinder3D~\cite{zhu2021cylindrical} &   \xmark         &        &        &        &        &                          \\

\specialrule{1.5pt}{0pt}{0pt}
\end{tabular}}
\end{table*}
